Effective Prime Factorization via Quantum Annealing by Modular Locally-structured Embedding

This paper investigates novel techniques to solve prime factorization by quantum annealing (QA). Our contribution is twofold. First, we present a novel and very compact modular encoding of a binary multiplier circuit into the Pegasus architecture of current D-Wave QA devices. The key contribution is a compact encoding of a controlled full-adder into an 8-qubit module in the Pegasus topology, which we synthesized offline by means of Optimization Modulo Theories. This allows us to encode up to a 21*12-bit multiplier (and a 22*8-bit one) into the Pegasus 5760-qubit topology of current annealers. To the best of our knowledge, these are the largest factorization problems ever encoded into a quantum annealer. Second, we have investigated the problem of actually solving encoded PF problems by running an extensive experimental evaluation on a D-Wave Advantage 4.1 quantum annealer. In order to help the annealer in reaching the global minimum, in the experiments we introduced different approaches to initialize the multiplier qubits and adopted several performance enhancement techniques. Overall, exploiting all the encoding and solving techniques described in this paper, 8, 219, 999 = 32, 749 * 251 was the highest prime product we were able to factorize within the limits of our QPU resources. To the best of our knowledge, this is the largest number which was ever factorized by means of a quantum annealer, and, more generally, by a quantum device.

==> iteratedRV.tex <==
\subsection*{\color{red} Solving PFs with iterated reverse annealing}


\ignore{
After conducting an analysis of the Hamming distance between the minima attained through both forward annealing (with pauses) and reverse annealing (with pauses), as depicted in Figure \ref{tab: large_factoring}, it has been observed that in the majority of cases where the global minimum is ultimately achieved through the reverse annealing process, the former forward annealing provides a {\it good} state, 
i.e., close to the global minima with a Hamming distance of approximately 20.
However, this is not always the case: there are some problem instances for which the forward-then-reverse process fails to find the global minima despite a good starting point for reverse annealing.
In this section, we investigate whether a series of consecutive reverse annealing processes (from now on referred as \textit{Iterated Reverse Annealing (IRV)}) from good forward annealing results,
can positively affect the probability of reaching the global minimum.
}

\ignore{
If we compare the Hamming distance between the minima attained through forward annealing against reverse annealing (i.e. the number of variables having different truth values among the two minima), we observe that in the majority of cases where the global minimum is ultimately achieved through reverse annealing, the former forward annealing provides a {\it good} state, 
i.e., close to the global minima with a Hamming distance of approximately less than 20. A factor that could affect the probability of reaching a ground state through reverse annealing is thermal relaxation through pauses, possibly leading to better performances of reverse annealing even with higher Hamming distances. To this extent, we investigate whether a series of consecutive reverse annealing processes with different pauses (from now on referred to as \textit{Iterated Reverse Annealing (IRV)}) can positively affect the probability of reaching the global minimum.
}

One factor that heavily influences the results obtained from the two-quantum search described in the previous section is the . Depending on the 

\ignore{
IRV begins with the minimum
obtained by pure forward annealing without pausing,
excluding the impact of thermal fluctuation 
on the distance of the state to the global minima;
in the following iterations, it will trasverse newly obtained whole lower-energy space
to explore more paths for reaching the desired global minima.
For each state from which the RV starts,
a set of pause times will be considered, e.g., $T_p \in \{1, 10, 30, 50, 100\}\mu s$.
Note that the longer the pause time is, the greater role the thermal fluctuation comes to play.
Manifested in the movements in search space, 
the longer pause time extends the RV inversion point
where large movements are possible to drive.
In this IRV, the consideration of the pause time
terminates once a lower-energy state is obtained,
for the sake of saving QPU time.
}

IRV consists of planning a set of reverse annealing processes with different pausing times from a non-ground state obtained from a forward annealing process. Longer pauses increase the probability of reaching a ground state, but require plenty of high-cost resources. For this reason, we start from low values of pausing, seeing if the state obtained from reverse annealing has a lower energy than the initial state from forward annealing. If this is the case, then we can interrupt IRV and check the satisfiability of the current state. In the case the state from reverse annealing has a higher energy or a lower energy bit still does not correctly factorize the input number, we move on to the next process planned by IRV, further increasing the effect of thermal relaxation. Otherwise, the reverse annealing has correctly factorized the prime number and we stop the search, avoiding running additional reverse annealing processes.

We tested IRV on $12\text{bit}\times 8\text{bit}$,
$14\text{bit}\times 8\text{bit}$,
and $16\text{bit}\times 8\text{bit}$ factorization problems that were not solved by previous approaches, using the improved CFA encoding shown in Figure \ref{fig: unify} and initializing qubits setting flux biases. Our novel technique succeeds in finding the global minimum
for the $12\text{bit}\times 8\text{bit}$
and $14\text{bit}\times 8\text{bit}$ instances 
after 2 and 4 iterations, respectively. Even though the $16\text{bit}\times 8\text{bit}$ factorization problem has not been solved in four iterations, we notice the sample energy rapidly gets closer to zero the more processes are planned by IRV.

\ignore{
The approach for factoring a number of
$12\text{bit}\times 8\text{bit}$,
$14\text{bit}\times 8\text{bit}$,
and $16\text{bit}\times 8\text{bit}$
on DWave Advantage 4.1,
using the improved CFA encoding shown in Figure \ref{fig: improved_CFA1},
together with the initialization via flux bias.
The IRV succeeds in finding the global minima
for the $12\text{bit}\times 8\text{bit}$
and $14\text{bit}\times 8\text{bit}$ instances 
after two and four iterations respectively,
as shown in Table \ref{tab: IRV}.
The occurrance of the obtained global minima,
out of 1000 samples with $T_a =20\mu s$,
is denoted in $[]$.
These results confirm that IRV is effective
in finding global minima
if it can be iteratively initialized in a reasonable state.
In our case, this state is not necessary the minima
instead a state of little higher energy.
This works under the umbrella of gradually 
closer-to-global-minima and suppressed search space,
which is implemented by finding the {\it optimal} inversion point
out of a chosen region, e.g., $Sp \in [0.3, 0.4)$,
for each pause time, 
i.e., the point where RV could drive the system to a new-lowest-energy state.
The efficency of this Breadth-First-Search (BFS)-like IRV 
depends on the size of obtained lower-energy space in each iteration;
moreover, the choice of the pause times and inversion point in each iteration of IRV
determines the Hamming distance the system can move 
through reverse annealing, impacting accessiable search space.
Therefore, a suitable choice of pause times in each iteration of IRV is expected to improve
the efficienty of this IRV.
}


\begin{table}
\begin{tabular}{|l|l|c|c|c|c|}
\toprule
\multirow{2}{*}{size} & \multirow{2}{*}{$P= A\times B$} 
& \multicolumn{4}{c}{$(minima, T_p, S_p, new\ minima)$}\\
	 &                & 1 & 2 & 3 & 4 \\
\midrule
$12\times 8$ & $1027343=4093\times 251$
& (10.167, 1, 0.31, 6.167) & (10.167, 1, 0.38, 4.083) & (4.083, 100, 0.38, 0[2]) & - 
\\
\midrule
$14\times 8$ & $4111631=16381\times 251$
& (18.167, 1, 0.35, 8.083) & (16, 1, 0.35, 6) & (10, 50, 0.37, 2.083) & (2.083, 10, 0.38, 0[67])
\\
\midrule
$16\times 8$ & $16445771=\text{unknowns}$
& (18.333, 1, 0.34, 6.083) & (10, 10, 0.35, 4) & (6.083, 50, 0.36, 4.167) & (4, 100, 0.39, 4)\\
\bottomrule
\end{tabular}
\caption{\label{tab: IRV} Results of IRV,
with the multiplier encoded by the improved CFA shown in Figure \ref{fig: improved_CFA1}
and initialized via flux bias}
\end{table}
